Memory-efficient Speech Recognition on Smart Devices

Recurrent transducer models have emerged as a promising solution for speech recognition on the current and next generation smart devices. The transducer models provide competitive accuracy within a reasonable memory footprint alleviating the memory capacity constraints in these devices. However, these models access parameters from off-chip memory for every input time step which adversely effects device battery life and limits their usability on low-power devices. We address transducer model's memory access concerns by optimizing their model architecture and designing novel recurrent cell designs. We demonstrate that i) model's energy cost is dominated by accessing model weights from off-chip memory, ii) transducer model architecture is pivotal in determining the number of accesses to off-chip memory and just model size is not a good proxy, iii) our transducer model optimizations and novel recurrent cell reduces off-chip memory accesses by 4.5x and model size by 2x with minimal accuracy impact.

==> accuracy.tex <==
\section{Efficiency vs Accuracy Tradeoff}
\label{sec:accuracy}

In this section, we train the desirable networks from the previous section to understand their accuracy potential. We compare:
\begin{itemize}
    \item Shallow vs Deep Encoder. \textbf{Desired outcome:} accuracy of the deep encoder is comparable/better than shallow ones.
    \item Sparse vs Dense recurrent path in encoder. \textbf{Desired outcome:} accuracy of sparse recurrent path comparable/better than dense. 
    \item Subsampling vs smaller encoder. Neutral.
    \item Shallow vs Deep Decoder. \textbf{Desired outcome:} Decoder amenable to some depth increase.
\end{itemize}

==> analyticalModel.tex <==
\section{Analytical Modeling of Efficiency}
\label{sec:analytical}

\begin{table*}[ht]
\begin{varwidth}[b]{0.6\linewidth}
%\begin{center}
\caption{Memory Cost Model: Parameter Access Count with on-chip caching enabled}
\label{tab:memcost}
%\vskip 0.15in
\resizebox{\linewidth}{!}{%
%\begin{small}
\begin{sc}
\begin{tabular*}{1.5\linewidth}{lcccr}
\toprule
Component & Parameter & Access Count & Working Set & Note \\
\midrule
Encoder   & $W_{ih}$  & $\frac{|W_{ih}|}{C}$ & 0 & ``C'' time steps\\
Encoder   & $W_{hh}$  & $\frac{|W_{hh}|}{C}$ & $|W_{hh}|$ & ``C'' Matrix-vector ops\\
Decoder   & $W_{ih}$  & $\frac{|W_{ih}|}{C_d}$ & $|$Decoder + Prediction$|$ & $C_d$ symbols decoded  \\
Decoder   & $W_{hh}$  & $\frac{|W_{hh}|}{C_d}$ & $|$Decoder + Prediction$|$ & $C_d$ symbols decoded  \\
\bottomrule
\end{tabular*}
\end{sc}
}
%\end{small}
%\end{center}
\vskip -0.3in
\end{varwidth}
\hfill
\begin{minipage}[btm]{0.4\linewidth}
 \centering
\includegraphics[width=0.85\columnwidth]{figures/hwAbstract}
 \captionof{figure}{Hardware Abstraction and Energy Model}
 \label{fig:hwmodel}
 \vskip -0.3in
\end{minipage}
\end{table*}

In this section, we discuss our approach for estimating the efficiency of a transducer model. The goal is to identify model architectures that can execute efficiently on mobile devices without overly specializing the exploration to a particular SoC or software library. We first overview an abstract hardware design that guides our cost model. Next we discuss a metric to quantify the cost of a transducer model (inverse of efficiency).

\subsection{Hardware Abstraction}
\label{sec:hardware}

This section presents a simple high-level hardware model that abstracts away much of the implementation details of mobile SoCs while capturing the fundamental properties of the different hardware structures.  Our model, shown in Figure~\ref{fig:hwmodel}, just consists of compute, on-chip buffer and memory. 
\begin{description}
	\item[Compute units:] These are the arithmetic building blocks such as multiply-accumulate (MAC) units. 
	\item[Memory:] This is the high capacity main memory where all the models reside and are accessed from to perform an inference. In terms of per-access cost, memory is two orders of magnitude more expensive than computation.
	\item[On-chip Buffers:] These are temporary data buffers (scratchpads or caches) that helps amortize the cost of accessing data from memory by reusing them across many computations. However, to leverage on-chip buffers, the working set of the computation must be smaller than the on-chip buffer. 
\end{description}
We chose this model instead of an hardware instance-specific evaluation because the mobile architecture is rapidly changing with new hardware features being added (or explored) for neural architecture~\cite{iphonenpu,huaweinpu,googleetpu,asrdb,epurlstmaccl} and an easy to reason about analytical model would be more useful and reusable. Furthermore, this sort of model aligns well with first order cost models~\cite{dlacclsurvey} used in new accelerator explorations. As a result, for first order analysis, we believe this is a good trade-off that allows us build hardware-friendly models while not over-specializing to any one hardware implementation.


\boldparagraph{Baseline Network Energy Profile:} We show the energy breakdown using this model for our baseline transducer network (described in Section~\ref{sec:efficiency}) in Figure~\ref{fig:hwmodel}. The total energy is dominated by the memory accesses -- this is because of limited data reuse and the models being too large to benefit significantly from on-chip buffers. This is in keeping with the findings of the prior work in this domain~\cite{lstmmempower1,lstmmempower2}.  To address this,  we look at neural architecture variations that improve the memory access efficiency unlike the prior work that focuses primarily on  reducing the model size.

\begin{figure}

\end{figure}

\subsection{Model Cost} 
\label{sec:modelcost}

Two common dimensions along which one can quantify the cost of a neural network model are as follows:
\begin{description}
	\item[Computation:] This approach just sums up all the MACs needed to compute an output. While a popular cost metric for computationally heavy CNN models, this metric is not be very relevant for recurrent transducer models because they are dominated by memory accesses. 

	\item[Model Size:] This metric uses the total number of parameters in a model. This is a commonly used metric for models that are limited by memory capacity of the deployed systems or limited by memory bandwidth. The recurrent transducer model for speech do not suffer from memory capacity issues because of their end-to-end nature and doing away with the memory heavy external language model. Moreover, for transducer networks, total model size is not a reliable indicator of whether the network will be memory bandwidth bound. This is because only part of the network (encoder or prediction) is used at any given moment. Also, the different components vary in their ability to leverage the hardware optimization of having on-chip SRAMs to increase the reuse of the data fetched from the main memory.   
\end{description} 

\boldparagraph{Memory Cost Model: Parameter Access Count under the working set constraint of a cache-able parameter count, $W_{buf}$.} To account for the unique characteristics of the recurrent transducer models, we consider an alternate metric: average number of accesses to the model parameters after taking into account any potential parameter data reuse that can be realized with on-chip SRAM $\le W_{buf}$. This metric focuses on the memory access count for model parameters which dominate the performance and energy of a recurrent transducer model and does so by taking into consideration the model size, execution schedule and on-chip caching. Concretely, Table~\ref{tab:memcost} shows the average memory access cost of the different components of a recurrent transducer model and the amount of working set needed to capture the reuse. 
\begin{description}
    \item[Encoder - $W_{ih}$:] Encoder's input-to-hidden path is the easiest to optimize in terms of reusing parameters fetched from memory. This reuse is proportional to the number of time steps we can batch within the system's latency constraints. 
    \item[Encoder - $W_{hh}$:] Encoder's hidden-to-hidden path needs to run sequentially and can realize parameter reuse only if the whole weight matrix for a layer fits in on-chip buffer. Hence, they can benefit significantly from  on-chip buffer.
    \item[Prediction - $W_{ih}$, $W_{hh}$:] Given the auto-regressive nature of transcription, we can achieve reuse for the weights only if a complete decoder layer fits on-chip. This significantly limits the benefit of on-chip caching for the decoder path. We assume $C_d$ is 1 in our studies to model the  streaming mode.
\end{description}


==> efficiency.tex <==
\section{Model Architecture Efficiency Exploration}
\label{sec:efficiency}

\info[inline]{
Plan for this section:	
\begin{itemize}
	\item Iso-size encoder variation of layer size vs encoder depth to show config matters.
	\item Vary the encoder hidden state size
	\item Vary the number of layers 
	\item Iso-size decoder variation of layer size vs decoder depth to show config does not matter much.
	\item Impact of beam search on execution efficiency
	\item Complete model with varying encoder and decoder
	\item Validate findings against kernels running on HiFi DSP
\end{itemize} 
}


This section plots the efficiency impact of different network design options. We first look at the different design options for the encoder network and prediction network separately. Next we look at how to put them together into an efficient recurrent transducer network. For this analysis, we consider the following system design points:
\begin{description}
	\item[\ibs: Input timestep batching factor of 8] Targets low-latency transcription.
	\item[\ibl: Input timestep batching factor of 32] Tolerates lag in transcription.
	\item[\wss: Working set size of 500K params] Limited on-chip storage.
	\item[\wsl: Working set size of 2M params] Sizable on-chip storage to optimize for memory.
\end{description}

Finally we end the section with some validation analysis where we correlate the findings from our analytical model to the behavior of the compute kernels on a DSP.


\info[inline]{Graph: X-Axis: dimension being explored. Y-Axis: Normalized growth of compute and memory access count. }

\change[inline]{Make all the graphs pretty and comprehensible. Just placeholders for now to look at the data.}

\subsection{Encoder Network}
\label{sec:encoderResult}
\begin{figure*}
 \centering
\includegraphics[width=\columnwidth]{graphs/encIsoModelHiddenState.png}
\includegraphics[width=\columnwidth]{graphs/encIsoModelDepth.png}
\includegraphics[width=\columnwidth]{graphs/encHiddenStateScaling.png}
\includegraphics[width=\columnwidth]{graphs/encDepthScaling.png}
 \caption{Encoder scaling experiments. Top Graphs: Iso-model size by varying hidden state and depth. Bottom graphs: Increasing model size by increasing the hidden state (left) or the network depth (right).}
 \label{fig:encScaling}
\end{figure*}

As we discuss in section~\ref{sec:encoder}, the behavior of the encoder network is controlled by the per-layer weight size, number of layers and the subsampling factor across the encoder layers. Figure~\ref{fig:encScaling} shows the impact of scaling the layer width and depth on the compute-to-byte ratio as well as total memory accesses. The top figure shows that even for the same model size, the encoder configuration has a non-trivial impact on the memory access efficiency of the network. 

\subsection{Prediction Network}
\label{sec:predResult}

\subsection{Recurrent Transducer Network}
\label{sec:rnntResult}

\subsection{Analytical Model Validation}
\label{sec:validation}

In this section, we correlate the findings of our analytical model with the behavior of matrix vector and matrix-matrix kernels on the HiFi DSP.

==> efficiencyV2.tex <==
\section{Optimizing Transducer Models}
\label{sec:efficiency}

\begin{figure}
 \centering
\includegraphics[width=0.9\columnwidth]{graphs/memAccessCompare.pdf}
\vskip -0.1in
 \caption{Memory Access Breakdown (normalized to baseline) for recurrent transducer model variations. }
 \label{fig:memAnalysis}
 \vskip -0.22in
\end{figure}

In this section, we first present the cost of an inference with transducer model -- focusing on the memory access count since they account for majority of the energy (Section~\ref{sec:analytical}). Then we discuss optimizations to improve memory efficiency. 

\boldparagraph{Dataset:} We use a  video dataset  sampled from publicly shared English videos~\cite{englishviddataset}. The data is completely anonymized; both transcribers and researchers do not have access to any user-identifiable information (UII). Training set consists of 941.6K videos or 13.7K hours in length. The average video is 52.6 seconds long with a standard deviation of 45.9 seconds. Test dataset consists of 1.4K/20.9 hrs videos (\emph{vid-clean}). It contains a diverse set of speakers, content types, and acoustic conditions. For simpler/faster training flow, we did not use known  techniques such as Layer Norm or pre-training that can improve  WER~\cite{rnnt,rao2018exploring,lcblstmmj} by multiple points. We expect all our model variations to benefit from these techniques.
%\todo{check table caption}
\begin{table}[htbp]
\caption{Optimizations used for different network components and the corresponding memory access savings}
\label{tab:rnntopt}
\vskip -0.1in
\centering
%\begin{small}
%\begin{sc}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccc}
\toprule
ID & Component & Optimization & Savings \\
\midrule
Sched & Encoder $W_{ih}$ & Timestep batching (Section~\ref{sec:timebatch}) & ~\concern{4$\times$} \\
Residual & Encoder $W_{hh}$ & Persistent RNN (Section~\ref{sec:prnn}) & ~\concern{5$\times$} \\
SRU & Decoder & SRU (Section~\ref{sec:sru}) & ~\concern{2.1$\times$} \\
\bottomrule
\end{tabular}
%\end{sc}
%\end{small}
}
\vskip -0.1in
\end{table}


\subsection{Baseline Network Model}
\label{sec:baseline}
%\improvement[inline]{Add more info about the network and also discuss the dataset}
Our baseline model uses 4-layer, 1280 hidden units encoder and 2-layer, 1024 hidden units prediction network. In the default execution schedule, the network executes one time frame at a time. The corresponding memory cost breakdown is shown in Figure~\ref{fig:memAnalysis} as the ``Baseline'' bar. As we expect, the encoder accounts for the vast majority of the memory accesses. Furthermore, the input path and the recurrence path account for almost the same number of memory accesses.

One network optimization is subsampling~\cite{las} the time frames as we go deeper in the encoder network -- this helps with training convergence and  reduces the compute requirement. In our model, we subsample twice to help with network convergence. We show the memory cost of this model in Figure~\ref{fig:memAnalysis} as "Baseline-sub" -- it is ~\concern{1.3$\times$} fewer accesses.

\subsection{Scheduling Encoder Input-to-Hidden Path}
\label{sec:timebatch}


In this section, we discuss reordering encoder's LSTM computation across the time steps to improve the memory access efficiency of $W_{ih}$ parameters. As we discuss in Section~\ref{sec:rnnt}, multiple input vectors -- $X_is$ -- are  available in parallel during inference. One approach to improve the memory access efficiency of  $W_{ih}$  is to use them for multiple input vectors, say `B' of them as shown in Figure~\ref{fig:rnntSched}. The amount of reuse, B, depends primarily on our tolerance to latency between speech and text output. For example, if B is 8, then we batch 8 time steps and feed them through the encoder layer. This can introduce up to 160 ms of latency -- 80 ms for the initial batching and worst case real-time factor of 1. We use B = 8 in our experiments to model a low-latency transcription and that leads to \concern{1.4$\times$} memory access savings (Figure~\ref{fig:memAnalysis}, Sched Opt bar).  
\begin{figure}[!tb]
 \centering
\includegraphics[width=0.85\columnwidth]{figures/rnntTimeBatching}
 \caption{RNN Transducer Encoder Scheduling Options}
 \label{fig:rnntSched}
 \vskip -0.2in
\end{figure}

\boldparagraph{Computation Scheduling with Time Batching:} In a standard LSTM cell, we have four gates where each gate uses a matrix-vector followed by non-linearities. We can decompose this matrix-vector into two operations -- one on the input vector ($x_t$) and second using hidden state ($h_t$). We can fetch $W_{fi}$, $W_{Ci}$, $W_{ii}$, $W_{oi}$ only once and apply it to multiple $x_t$, making them batchable. In Figure~\ref{fig:rnntSched}, the batchable operations are shown in blue and non-batchable in red.
\begin{equation*}
\begin{split}
\begin{bmatrix}
    W_f \\ W_i \\ W_C \\ W_o
  \end{bmatrix}\cdot \begin{bmatrix}
    h_{t-1} \\ x_t 
  \end{bmatrix} & = \begin{bmatrix}
    W_{fh} \\ W_{ih} \\ W_{Ch} \\ W_{oh}
  \end{bmatrix}\cdot h_{t-1} + \begin{bmatrix}
    W_{fi} \\ W_{ii} \\ W_{Ci} \\ W_{oi}
  \end{bmatrix}\cdot x_{t} \\
  &= \underbrace{W_{hh}\cdot h_{t-1}}_{non-batchable}+\underbrace{W_{ih} \cdot x_t}_{batch\textmd{ }across\textmd{ }t}
\end{split}
\end{equation*}
% \begin{equation}
% W_f\cdot[h_{t-1},x_t] = \underbrace{W_{fh}\cdot h_{t-1}}_{non-batchable} +   \underbrace{W_{fi}\cdot x_t}_{batchable}
% \end{equation}
% \begin{equation}
% W_i\cdot[h_{t-1},x_t] = \underbrace{W_{ih}\cdot h_{t-1}}_{non-batchable} +   \underbrace{W_{ii}\cdot x_t}_{batchable} 
% \end{equation}
% \begin{equation}
% W_C\cdot[h_{t-1},x_t] = \underbrace{W_{Ch}\cdot h_{t-1}}_{non-batchable} +   \underbrace{W_{Ci}\cdot x_t}_{batchable}
% \end{equation}
% \begin{equation}
% W_o\cdot[h_{t-1},x_t] = \underbrace{W_{oh}\cdot h_{t-1}}_{non-batchable} +   \underbrace{W_{oi}\cdot x_t}_{batchable} 
% \end{equation}
\subsection{Encoder Hidden-to-Hidden Path}
\label{sec:prnn}

This section looks at reducing the memory access count of the recurrent path using the persistent  RNN~\cite{persistentrnn} technique -- idea being to fetch the weights on-chip once and reuse it multiple times in sequence. Concretely, we fetch $W_{hh}$ of one encoder layer into on-chip buffer and reuse it `B' (time batch size) times. While this optimization provides significant savings (B$\times$), it relies on the recurrent weight matrix fitting on-chip. 

\boldparagraph{Optimizing required on-chip storage:} An approach we explore to reduce the size of the on-chip buffers required to capture $W_{hh}$ reuse is building narrow, deep models instead of wide, shallow models for the encoder. However, these deeper models introduce convergence issues with vanilla LSTM cells. We address this using Residual LSTM~\cite{rlstm} -- they allow us to build narrow, deep models without hurting accuracy. Table~\ref{tab:residualacc} shows that we can reduce the per-layer size of $W_{hh}$ without hurting accuracy by going to deeper networks. Furthermore, this improves memory efficiency by ~\concern{2.5$\times$} at the network level (Residual opt in Figure~\ref{fig:memAnalysis}).
\begin{table}[htbp]
\caption{Accuracy vs Depth in Transducer Networks}
\label{tab:residualacc}
\vskip -0.1in
\centering
%\begin{small}
%\begin{sc}
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{cccc}
\toprule
Hidden State & Depth & Parameters (M) & WER \\
\midrule
1280 & 4 & 6.25 & 22.17 \\
1024 & 8 & 4 & 21.7 \\
768 & 12 & 2.25 & 21.4 \\
\bottomrule
\end{tabular}
%\end{sc}
%\end{small}
%}
\vskip -0.1in
\end{table}


\subsection{ Prediction Network}
\label{sec:sru}



Unlike the encoder network whose execution provides us scheduling flexibility (along the time dimension vs the along the depth), the prediction network's autoregressive nature forces us to execute along the depth dimension. As a result, the only way to optimize the number of memory accesses in the decoder is reduce the number of parameters in the decoder. There are multiple techniques one can consider to reduce the parameter count -- LSTM variants such as projection lstm~\cite{lstmp}, simplified recurrent units (SRU~\cite{sru}) or optimizations such as weight pruning~\cite{lstmpruning1,lstmpruning2}. 

\begin{table}[htbp]
\caption{Accuracy of SRU Decoder in Transducer Networks. Encoder and Decoder columns show \emph{hidden state size} and \emph{depth}. \emph{Mem cost} captures savings in decoder memory access.}
\label{tab:sruacc}
\vskip -0.1in
\centering
%\begin{small}
%\begin{sc}
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
Model Arch & Encoder & Decoder & WER & Mem Cost \\
\midrule
Baseline & 1280, 4 & 1024, 2 & 22.17 & 1x\\\hline
Residual & 768, 12 & 1024, 2 & 21.40 & 0.96x\\\hline
SRU & 1024, 6 & 1024, 2 & 21.00 &  \\
 & 1024, 8 & 1024, 2 & 21.80 & \\
 & 768, 12 & 768, 2 & 21.43 & 0.45x\\
\bottomrule
\end{tabular}
%\end{sc}
%\end{small}
%}
\vskip -0.1in
\end{table}

In this work, we evaluate using SRU for the decoder layers where input and hidden state are the same size (to support residual without additional scaling) -- SRUs have smaller memory footprint, are computationally simpler and have shown to have similar/better accuracy as LSTMs. They provide good accuracy for recurrent transducer models  (Table~\ref{tab:sruacc}) while saving ~\concern{2.1$\times$} of decoder's memory accesses.\\

\boldparagraph{Summary:} Taken together, our network modifications reduce the memory accesses by ~\concern{2.8$\times$} on top of a compact and execution optimized transducer model ("Sched Opt" in Figure~\ref{fig:memAnalysis}).   

%%%%%%%%%%%%%%%%%%%% BIT BUCKER %%%%%%%%%%%%%%%
\ignore{
\begin{align*}
f_t &= \sigma(W_f\cdot[h_{t-1},x_t]^T+b_f)\\
i_t &= \sigma(W_i\cdot[h_{t-1},x_t]^T+b_i) \\
\tilde{C_t} &= tanh(W_C\cdot[h_{t-1},x_t]^T+b_C) \\
o_t &= \sigma(W_o\cdot[h_{t-1},x_t]^T+b_o) \\
C_t &= f_t*C_{t-1} + i_t*\tilde{C_t}\\
h_t &= o_t*tanh(C_t)\\
\end{align*}
\vskip -0.1in
}
\ignore{We can decompose matrix-vector multiplication in $W_f\cdot[h_{t-1},x_t]$, $W_i\cdot[h_{t-1},x_t]$, $W_C\cdot[h_{t-1},x_t]$ and $W_o\cdot[h_{t-1},x_t]$ into two partial sums:}


==> intro.tex <==
\section{Introduction}
\label{intro}
\comment{Capturing the flow using bullet points. Need to write this out as a proper section in the future}

\begin{itemize}
	\item \textbf{Shared Context:} On-device ASR increasingly important. RNNT a promising class of models that achieve good accuracy with a small model size and no external LM.
	\item \textbf{Problem:} Little insight into how different network architecture configurations and sizing impacts the efficiency and accuracy of the model.
	\item \textbf{Problem Cost:} Inefficient, power-efficient execution on the edge devices leading to greater power and latency for the target accuracy.
	\item \textbf{Contribution:}
	\begin{enumerate}
		\item Network architectural knobs and how they impact on-device execution efficiency.
		\item Network architectural tricks to help train the efficient ones.
		\item Efficiency vs Accuracy analysis to understand the pareto-optimal curve.
	\end{enumerate}
\end{itemize}

\boldparagraph{Paper Outline:} The rest of the paper is organized as follows -- Section~\ref{sec:rnnt} overviews recurrent transducer model for speech recognition. Section~\ref{sec:analytical} presents our approach for analyzing the efficiency of the transducer models. Section~\ref{sec:efficiency} analyzes the efficiency of transducer model as well as investigates accuracy of the efficient network variants. Section~\ref{sec:conclude} concludes the paper. 

==> related.tex <==
\section{Prior Work}
\label{sec:related}

There has been a number of recent efforts on improving the accuracy of end-to-end neural ASR models~\cite{rnnt,rnntopt1,rnntopt2,rnntopt3}. Our work complements these prior efforts in that we focus on the execution efficiency of end-to-end neural architecture. 

RNN Transducers~\cite{rnnt} demonstrated a performant end-to-end neural architecture model -- small enough to fit within a reasonable memory capacity, provides good accuracy for the general ASR problem, operates in a streaming fashion and supports personalization. There has been follow-on work~\cite{rnntperfopt} on optimizing the model size. While model size is a popular proxy for efficiency, as we show in section~\ref{sec:efficiency}, it is not a good proxy for execution efficiency and instead focus directly on memory access efficiency. 

Finally, there is work on automated neural architecture search techniques for attention-based speech recognition models and focuses on reducing the model size~\cite{shrinkml}. We hope to explore this direction in the future to focus directly on execution efficiency of streaming models.

\concern{Cite and talk about LSTM search odyssey}

==> relatedList.tex <==
\ignore{
\begin{enumerate}
    \item Before RNNT
    \item RNNT and forward
    \begin{enumerate}
        \item A bunch of work on improving the accuracy of end-to-end models to enable the streaming use case 
        \item Streaming End-to-end ASR focuses on reducing the model capacity. We look at making it memory efficient.
        \item Candidate work: Focuses on decreasing model size and we observe that it is not a good metric for performance or efficiency. We focus on component specific optimizations
        \item ShrinkML: Proposes AutoML for per-layer compression using SVD. Their approach is orthogonal to this approach and can be used to further improve our efficiency. They use model size as proxy for performance and note it is not a good metric. https://arxiv.org/pdf/1907.03540.pdf
    \end{enumerate}
\end{enumerate}
}
